Driving into the Future: Multiview Visual Forecasting and Planning with World Model for Autonomous Driving

In autonomous driving, predicting future events in advance and evaluating the foreseeable risks empowers autonomous vehicles to better plan their actions, enhancing safety and efficiency on the road. To this end, we propose Drive-WM, the first driving world model compatible with existing end-to-end planning models. Through a joint spatial-temporal modeling facilitated by view factorization, our model generates high-fidelity multiview videos in driving scenes. Building on its powerful generation ability, we showcase the potential of applying the world model for safe driving planning for the first time. Particularly, our Drive-WM enables driving into multiple futures based on distinct driving maneuvers, and determines the optimal trajectory according to the image-based rewards. Evaluation on real-world driving datasets verifies that our method could generate high-quality, consistent, and controllable multiview videos, opening up possibilities for real-world simulations and safe planning.

==> fig/CounterFactual.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{fig/counterfactual_v2.pdf}
    \caption{\textbf{Counterfactual events generation.} Top: turning around at a T-shape intersection on a rainy day. Note that our training set does not contain any turning-around samples. Bottom: running over a non-drivable area.}
    \label{fig:counter_factual}
    \vspace{-10pt}
\end{figure*}


==> fig/diverse_speed.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/diverse_speed.png}
    \caption{\textbf{Diverse speeding behaviors.} We input different patterns of speed signals into our model to assess controllability in terms of speed. The top series shows that the ego car decelerates and then accelerates while the bottom one shows a contrary behavior. These two results highlight the realism of our model's prediction.}
    \label{fig:diverse_speed}
\end{figure*}
 

==> fig/diverse_turning.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/diverse_turning.png}
    \caption{\textbf{Diverse turning behaviors.} Utilizing an identical initial frame, we provide our model with sequences of positive steering angles (indicating a left turn) and negative values (indicating a right turn). The figure demonstrates the model's proficiency in generating consistent street views for both turning behaviors. Each frame is accompanied by a blue bar, indicating the corresponding steering angle in degrees. A longer bar correlates with a more substantial steering angle. For clarity, only the front view is shown.}
    \label{fig:diverse_turning}
\end{figure*}
 

==> fig/multimodal_plan.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth]{fig/turn_left.pdf}
    \caption{Turn left.}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth]{fig/turn_right.pdf}
    \caption{Turn right.}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth]{fig/speed_up.pdf}
    \caption{Speed up.}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
    \includegraphics[width=\linewidth]{fig/slow_down.pdf}
    \caption{Slow down.}
    \end{subfigure}
    \caption{\textbf{Generation of Multiple Plausible Futures.} world model could generate plausible videos for multimodal driving plans(generated videos here)}
    \label{fig:multimodal plans}
\end{figure*}

==> fig/resampling.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{fig/data_distrib.png}
    \caption{\textbf{The ego-action distribution before (left) and after re-sampling (right).} We re-sample rare combinations of speeds and steering angles, obtaining a balanced training dataset.}
    \label{fig:resampling}
\end{figure*}
 
